Trans-IR Flows to Black Hole Singularities

We study analytic continuations of holographic renormalization group (RG) flows beyond their infrared (IR) fixed points. Such "trans-IR" flows are a natural framework for describing physics inside of black holes. First, we construct a monotonic holographic $a$-function which counts degrees of freedom along a trans-IR flow. Using this function, we argue that the degrees of freedom "thin out" and vanish when flowing to a trans-IR endpoint, represented by a Kasner singularity. We then recast well-studied quantum information probes in the language of trans-IR flows, finding that entanglement and complexity from volume generally fail to fully probe the trans-IR while 2-point correlations and complexity from action generally do so in a complementary manner.

==> todolist.tex <==
\begin{itemize}
\item[I.] \textcolor{blue}{Introduction}
\item[II.] \textcolor{blue}{The Monotonic $a_T$-Function}
\begin{itemize}
\item[A.] \textcolor{blue}{Defining the Function}
\item[B.] \textcolor{blue}{Proof of Monotonicity}
\end{itemize}
\item[III.] \textcolor{blue}{The Nature of the Singularity}
\begin{itemize}
\item[A.] \textcolor{green}{Numerical Construction of Kasner Flows}
\item[B.] \textcolor{blue}{Probing the Kasner Singularity} (Gubser criterion?)
\end{itemize}
\item[IV.] \textcolor{blue}{Euclideanization and Time in the Interior}
\begin{itemize}
\item[A.] \textcolor{blue}{Trans-IR Flow as Dynamical Evolution}
\item[B.] \textcolor{blue}{Trans-IR Flow as Euclidean State Preparaton}
\end{itemize}
\item[V.] \textcolor{blue}{Signals of Trans-IR in Quantum Information}
\begin{itemize}
\item[A.] \textcolor{blue}{Entanglement Entropy}
\item[B.] \textcolor{blue}{Holographic Complexity}
\begin{itemize}
\item[1.] \textcolor{green}{Complexity=Volume}
\item[2.] \textcolor{blue}{Complexity=Action}
\end{itemize}
\item[C.] \textcolor{blue}{Entanglement Negativity}
\end{itemize}
\item[VI.] \textcolor{blue}{Conclusions}
\item[A.] \textcolor{blue}{Null Hypersurfaces}
\end{itemize}
